Stochastic Market Games

Some of the most relevant future applications of multi-agent systems like autonomous driving or factories as a service display mixed-motive scenarios, where agents might have conflicting goals. In these settings agents are likely to learn undesirable outcomes in terms of cooperation under independent learning, such as overly greedy behavior. Motivated from real world societies, in this work we propose to utilize market forces to provide incentives for agents to become cooperative. As demonstrated in an iterated version of the Prisoner's Dilemma, the proposed market formulation can change the dynamics of the game to consistently learn cooperative policies. Further we evaluate our approach in spatially and temporally extended settings for varying numbers of agents. We empirically find that the presence of markets can improve both the overall result and agent individual returns via their trading activities.

==> Stochastic Market Games/content/0-abstract.tex <==
\begin{abstract}
Some of the most relevant future applications of multi-agent systems like autonomous driving or factories as a service display mixed-motive scenarios, where agents might have conflicting goals. In these settings agents are likely to learn undesirable outcomes in terms of cooperation under independent learning, such as overly greedy behavior. Motivated from real world societies, in this work we propose to utilize market forces to provide incentives for agents to become cooperative. As demonstrated in an iterated version of the Prisoner's Dilemma, the proposed market formulation can change the dynamics of the game to consistently learn cooperative policies. Further we evaluate our approach in spatially and temporally extended settings for varying numbers of agents. We empirically find that the presence of markets can improve both the overall result and agent individual returns via their trading activities.
\end{abstract}

==> Stochastic Market Games/content/1-introduction.tex <==
\section{Introduction}\label{sec:introduction}
In addition to the breakthroughs of multi-agent learning in fully cooperative domains  \cite{foerster2018counterfactual,rashid2018qmix,sunehag2018value}, recently more attention has been paid to multi-agent learning in mixed scenarios, where multiple self-interested agents live in a common environment \cite{dafoe2020open,hostallero2020inducing}. In mixed scenarios agents are characterized by general sum returns, so agents might compete or even have conflicting goals. These settings give rise to severe problems such as the tragedy of the commons \cite{ostrom1990governing,hardin2009tragedy,perolat2017multi}, and often lead to undesirable outcomes in the presence of learning, resulting in overly greedy or aggressive behavior \cite{leibo2017multi,lerer2017maintaining}. Humans on the other hand display the ability to overcome these pathologies through the evolution of social structures (also called institutions) \cite{ostrom1990governing,janssen2008turfs}, which renders the question of how known structures can be utilized or learned in the context of multi-agent systems.

\begin{figure}[hbtp]
\centering
\includegraphics[width=0.31 \textwidth]{img/SMG.pdf}
\caption{Stochastic Market Game: In addition to their environmental actions at time $t$, agents choose market actions, which are processed by a market function to compute agent specific rewards.}
\label{fig:SMG}
\end{figure}

Effective institutions shape the interaction of individuals, by setting constraints or providing specific incentives to the members of a society. Markets for instance are effective means to organize large numbers of self-interested entities in a decentralized manner, with a rich body of literature on markets dating back to Adam Smith \cite{smith1937wealth}. Besides its attributes of openness and scalability, as \cite{miller1988markets} note, a market is particularly effective in promoting efficient, cooperative interaction between heterogeneous participants because (idealized) markets define distinctive rules (property rights, unforgeable currencies, trademarks), such that being cooperative becomes a dominant strategy in the game theoretic sense. While markets have been suggested to coordinate distributed decision making in fully cooperative multi-agent systems \cite{miller1988markets,holland1985properties,chang2020decentralized}, in this work we adopt markets to change the dynamics of a given mixed-motive game to promote cooperation and make defective strategies less attractive.

%to solve the credit assignment problem \cite{baum1999toward} or to learn in partially observable Markov decision processes, \cite{kwee2001market}

%A trade in a market marks a Pareto improvement as it will generally make both trading partners better off. 

Our main argument is that modelling agents as market participants turns agents' self-interest from a flaw into a feature, as voluntary trades are Pareto improvements (in the absence of external costs) and hence direct the overall outcome towards the Pareto optimum of the solution space. We introduce markets for a given multi-agent problem by extending the formulation of Stochastic Games (or Markov Games) \cite{littman1994markov} with 1): a set of dedicated market actions that allow agents to become active in a given market, and 2): defining a function that redistributes rewards based on agents' market behavior. We term this a \textit{Stochastic Market Game}.

%We build on the foundations of idealized markets \cite{miller1988comparative} which are characterized by rules to are enforced by the environment such that agents cannot violate property rights, deceive other agents or trick the market.

%We call a Stochastic game with the above extensions a \textit{Stochastic Market Game (SMG)} and introduce two classes of markets for further evaluation: conditional markets and unconditional markets, which differ in the way transactions are defined.

%In an unconditional market, transactions of reward are triggered only in case certain conditions are fulfilled. This, for instance, allows agents to incentivize each other by suggesting specific actions which are rewarded in case of execution. In an unconditional market, transactions need not be bound to conditions, which allows agents to participate in other agents' returns, simply by buying and selling shares of their returns to each other. 

%As a concrete instance for a conditional market, we discuss so called action markets \cite{schmid2018action}, a market form that allows agents to trade actions for reward. Additionally, we propose the shareholder market as an instance of an unconditional market, which is inspired by stock markets. In this market form, agents can become corporate units by selling shares from their own return to other agents. Agents can participate in other agents' returns by holding these reward shares from others, just like a shareholder of a company.



==> Stochastic Market Games/content/2-related-work.tex <==
\section{Related Work}\label{sec:related-work}
\paragraph{Markets in cooperative games.}
First proposals for utilizing market forces to decentralize computationally complex tasks date back to \cite{miller1988markets,miller1988comparative}, with probably the first algorithm for cooperative multi-agent systems given in \cite{holland1985properties}, called the Bucket Brigade. The algorithm works on the basis of entities called classifiers, which are composed of a condition and an action. When the system state matches the condition of an entity, it computes a bid and the entity with the highest bid is allowed to push its specific action onto an execution queue. The bid is distributed among the previously active classifiers that led the system to the triggering condition, such that chains of rewards originate and learning may take place. \textit{Hayek machines} \cite{baum1999toward} extend the original Bucket Brigade by property rights (to act in the world) through agents which can invest in their own descendants, in order to profit from their offspring later. Market-based reinforcement learning (RL) as a means to learn in partially observable Markov Decision Processes (POMDPs) has been suggested in \cite{kwee2001market}, which is based on a variant of the Hayek machine with an added memory register that can be manipulated by agents with specific write actions. More recently, the idea of buying and selling the right to act in the world by individual agents has been taken up in \cite{chang2020decentralized} and combined with different RL algorithms to formalize a general framework for organizing a society of agents. In contrast to the approaches described above, the focus of this work lies in non-cooperative or mixed settings, where agents have individual goals. We therefore do not seek to solve the credit assignment problem with market mechanisms but suggest markets as a catalyst to allocate resources to agents in order to improve overall efficiency.

%The original algorithm suffered from the circumstance that there was no credit conservation law implemented, which made it possible to generate money out of nothing. Approaches that consider the conservation of credit are proposed in \cite{schmidhuber1987evolutionary}, where agents also bid for actions to be executed. 

%Work in the field of non-cooperative multi-agent systems has been focusing rather on methods to establish cooperation between agents \cite{kleiman2016coordinate,de2006learning}, e.g. by means of opponent modelling or via defining social preferences rather than modelling agents as utility maximizing market participants. 

\paragraph{Non-cooperative systems.}
In \cite{perolat2017multi}, multi-agent reinforcement learning is used to analyze the emergent equilibria for common-pool resource appropriation settings, for which game theoretic models predict the tragedy of the commons. In \cite{leibo2017multi}, sequential social dilemmas (SSDs) are introduced, which extend social dilemmas of game theory to better capture real world aspects, such as temporal extension and non-binary grades of cooperation. The idea of trading actions in SSDs for independent agents has been proposed in \cite{schmid2018action}, where it has been shown that the approach promotes cooperative strategies. However, the empirical evaluation has been limited to two agents. In this work, Stochastic Market Games are proposed, providing a general framework for agents to learn the distribution of rewards as a meta game. In this work, the action market is categorized as an instance of a conditional market and reevaluated with up to $16$ agents. More recently, \cite{lupu2020gifting} proposed gifting, a mechanism that allows agents to directly assign reward to other agents, used as a means to overcome the tragedy of the commons. The gifting mechanism is similar to the market approach, as it extends action spaces with designated gifting actions. However, it differs from the idea of a market, as there is no actual trading between agents based on a buying and selling offer.

%In this work, we extend the MARL problem with Stochastic Market Games, thereby going beyond its application as a mere simulation framework, in order to solve dilemmas that arise under self-interested learning in allocation problems. We build our testing environments on the basis of sequential social dilemmas (SSDs), as introduced by \cite{leibo2017multi}, which extend social dilemmas of game theory to better capture real world aspects, such as temporal extension and non-binary grades of cooperation. Whereas in \cite{leibo2017multi}, the focus lies in the observation that agent behavior can be controlled through environmental parameters such as resource abundance, in this work, we use the concept of SSDs to test the market hypotheses. 

%\begin{figure}[hbtp]
%\includegraphics[width=0.4\textwidth]{img/envs/coin-game.pdf}
%\caption{Matrix game version of the Coin game derived from the original Coin game as suggested in \cite{lerer2017maintaining}. Two agents $i$ and $j$ compete for two coins. When $i$ picks $j$'s designated coin, $j$ gets $-2$ but agents get $+1$ for picking any coin.}
%\label{fig:coin-game}
%\end{figure}

%Opponent modelling \cite{he2016opponent,raileanu2018modeling,everett2018learning} has also been applied to SSDs, such as in \cite{wang2018towards}, where a cooperation degree detection network was trained to identify the opponent's current level of cooperation. Based on the opponent's behavior, an agent can then select its own cooperation degree as best response. Another work with the aim of building an opponent model is  \cite{foerster2018learning}, where agents reason over the learning of other agents by an additional term within the learning rule. The authors demonstrate that the encounter of two such agents can lead to tit-for-tat, a strategy famous for its cooperativeness and robustness regarding exploitation from defectors. In this work, agents do not build an opponent model, nor does learning involve any kind of recursive or theory of mind \cite{rabinowitz2018machine} like reasoning. Rather, other agents are considered as part of the environment by individual agents, such that results can be understood as the emergent outcome of independently learning agents trying to adapt to an ever changing environment. Additionally, agents in this work do not communicate explicitly or share the same model during training. However, the way agents make offers can be understood as some form of communication. Though, in contrast to explicit models of communication such as in \cite{foerster2016learning}, where agents can backpropagate error derivatives, information in the presence of a market is transferred only indirectly via agents' trading activity.

%Other work in the field of SSDs aims at establishing cooperation between self-interested agents by incorporating social preferences such as inequity aversion into the model \cite{hughes2018inequity}, where it is shown that inequity-averse agents improve the temporal credit assignment problem and promote cooperation. 



==> Stochastic Market Games/content/3-background.tex <==
market-games\section{Background}
%\paragraph{Markov-Decision Processes}
%In case of a single learning agent, the problem can formally be described as a Markov-Decision Process (MDP), which is a tuple $(\mathcal S, \mathcal A, \mathcal T, R)$ where $\mathcal S$ is the state space, $\mathcal A$ is the action space, $ R: \mathcal S \times \mathcal A \times \mathcal S \to \mathbb R$ is the reward function and $\mathcal T: \mathcal S \times \mathcal A \to S$ is the transition function. The agent's goal is to learn an optimal policy $\pi$ that maximizes its expected return $\mathcal R_{t} := \sum^{\infty}_{t=1} \gamma^{t-1}R_{t}$ where $\gamma < 1$ is a discount factor \cite{sutton2018reinforcement}.

%The optimal policy of an MDP is undominated, i.e. there is no state from which any other policy can achieve a better expected, discounted return. The policy $\pi$ can be expressed as a function $\pi : \mathcal S \to \mathcal P(\mathcal A)$ that maps states to probability distributions over the available actions $\mathcal A$. 

%One way to learn a policy is to learn an action value function $Q : \mathcal S \times \mathcal A \to \mathbb R$ that gives the value of an action in a certain state and define a policy by selecting actions according to their action values. A popular way to learn the action value function is Q-learning, where an agent $i$ updates its values according to: $$Q_{i}(s, a) \leftarrow Q_{i}(s, a) + \alpha \big[ r_{i} + \gamma \max_{a' \in \mathcal A^{i}}  Q_{i}(s', a') - Q_{i}(s,a) \big]$$ where $\alpha$ is the learning rate and $\gamma$ is a discount factor. During training, exploration can be incorporated through so called epsilon greedy action selection, where an agent selects its optimal action according to its current $Q$-function with probability $1-\epsilon$ or a random action with probability $\epsilon$.

%In contrast to value-based approaches, policy gradient based methods do not learn a value function. They directly search the policy space for the optimal policy $\pi^{*}_{\theta}(a|s)$ with parameters $\theta$. The policy is usually represented by a deep neural network, which is trained using gradient descent on $\theta$. The theoretical foundation of these approaches is the policy-gradient theorem (\ref{eq:policy_gradient}), which states that the derivative of the expected reward is the expectation of the product of the reward and gradient of the log of the policy.
%\begin{equation}
%\label{eq:policy_gradient}
%   \nabla \mathbb{E}_{\pi_{\theta}} = %\mathbb{E}_{\pi_{\theta}}[R(\mathcal{\tau})\log{\pi_{\theta}(\tau)}]
%\end{equation} 
%Moreover, policy gradient methods generate training data by using the current policy and stochastically sampling from the action distribution. 

%A good compromise between both methods are actor-critic algorithms that aim to combine the best of both worlds. The actor is responsible for selecting the right actions, while the critic estimates the state value function, which is in turn used to criticize the actor's actions, resulting in a rich training signal. A widely used actor-critic approach is Proximal Policy Optimization (PPO)~\cite{schulman1707proximal}. It combats sensitivity to the choice of hyperparameters, a problem from which many on-policy methods suffer. This is achieved by avoiding drastic changes in the policy. The main idea is to penalize substantial deviations of the probability ratio (\ref{eq:prob_ratio}) from being $=1$.
%\begin{equation}
%    \label{eq:prob_ratio}
%    r_t(\theta) = \frac{\pi_{\theta}(a_t|s_t)}{\pi_{\theta_{old}}(a_t|s_t)}
%\end{equation} 
%This stabilizes training and has been shown to be successful across a variety of domains and tasks, such as real time strategy games~\cite{berner2019dota,vinyals2019grandmaster} and robotics~\cite{tan2018sim,andrychowicz2020learning}.

In this work we consider systems comprised of multiple independent agents formalized as a Stochastic Game $\mathcal{G}$ (also called Markov game) \cite{littman1994markov}, which is defined by a set of states $\mathcal S$, and a collection of action sets $\mathcal A_1,...,\mathcal A_N$, one for each agent in the environment. Given a current state and one action from each agent the next state of the environment is defined by the transition function $\mathcal P : \mathcal S  \times \mathcal A_1 \times...\times \mathcal A_N \to PD(\mathcal S)$ where $PD(\mathcal S)$ is the set of discrete probability distributions over $\mathcal S$. Each agent has a reward function $ r_i : \mathcal S \times \mathcal A_1 \times...\times \mathcal A_N \to \mathbb R$, that defines its goal. An agent tries to learn an optimal policy $\pi^{i}$ that maximizes its expected sum of discounted rewards (called return) $\mathcal R_{i,t} := \sum^{\infty}_{t=1} \gamma^{t-1}r_{i,t}$ with discount factor $\gamma < 1$ \cite{sutton2018reinforcement}. In this work we consider scenarios of mixed motives, which means agents' rewards are correlated to varying extents so depending on the situation their goals might be aligned or be in conflict \cite{dafoe2020open}. 

% \cite{zhang2019multi}
%\paragraph{Independent Learning (IL)}
To model learning, we utilize independent learning, a decentralized reinforcement learning (RL) approach where agents independently follow individual learning rules such as Q-learning or policy gradient methods. With \emph{deep} RL each agent's policy is represented as a deep neural network denoted $\pi^{i}_{\theta}$ where $\theta$ are the trainable parameters of a neural network. Independent learning is popular in mixed motive scenarios, as no assumptions on each agent's goal are required during training. One drawback of this this paradigm is that agents implicitly model other agents as being part of the environment so in general IL suffers from the issue of non-stationarity (agents have a moving target). In practice non-stationarity can be mitigated by letting agents adapt to a slowly changing data distribution which stabilizes learning \cite{leibo2017multi}. 

\paragraph{Independent Deep-Q-Networks (IDQN).} IDQN models each agent $i$ as a an instance of a \textit{Deep-Q-Network (DQN)} \cite{mnih2015human}, gathering its own experience represented as tuple $(s, a, r, s')$ comprising a state $s$, an action $a$, a reward $r$ and a next state $s'$. At each training step a minibatch of transitions is sampled to update the state-action value function  $Q_{i} : \mathcal{S} \times \mathcal{A}_{i} \to \mathbb R $ according to the update rule: $Q_{i}(s, a) \leftarrow Q_{i}(s, a) + \alpha \big[ r_{i} + \gamma \max_{a' \in \mathcal A^{i}}  Q_{i}(s', a') - Q_{i}(s,a) \big]$ where $\alpha$ is the learning rate. From $Q_i$ a policy is derived by selecting actions according to their $Q$-values in a given state or (to encourage exploration) randomly with probability $\epsilon$.


%\begin{figure}[hbtp]
%\centering
%\includegraphics[width=0.2\textwidth]{img/decentralized-setting.pdf}
%\caption{In a fully decentralized setting, agents receive local observations from the environment, without explicit communication or sharing of information between agents.}
%\label{fig:decentralized-setting}
%\end{figure}

\paragraph{Independent Actor-Critic (IAC).}
With IAC each agent is modelled as an instance of an actor-critic algorithm. Actor-critic algorithms seek to learn optimal policies by combining value function learning with policy gradient based methods. The difference of policy based methods and value based methods is, that policy based methods directly search the policy space for the optimal policy $\pi^{*}_{\theta}(a|s)$ with parameters $\theta$. Here we utilize Proximal Policy Optimization (PPO)~\cite{schulman1707proximal}, an algorithm that ensures policy updates are relatively small to mitigate the negative effects associated with drastic changes in the policy. PPO achieves this by keeping the probability ratio
$r_t(\theta) = \frac{\pi_{\theta}(a_t|s_t)}{\pi_{\theta_{old}}(a_t|s_t)}$ close to $1$ with a clipped surrogate loss.


%The actor represents the policy, i.e. is responsible for selecting the right actions, while the critic estimates the state value function, which is in turn used to criticize the actor's actions, resulting in a rich training signal. 


%This stabilizes training and has been shown to be successful across a variety of domains and tasks, such as real time strategy games~\cite{berner2019dota,vinyals2019grandmaster} and robotics~\cite{tan2018sim,andrychowicz2020learning}. 
%For independent training of PPO, each agent is represented by an individual instance of PPO, with updates being done only on agent's individual observations and rewards.


==> Stochastic Market Games/content/4-approach.tex <==
\section{Stochastic Market Games}\label{sec:approach}
In situations of mixed-motives, in which agents' interests are possibly conflicting, a central hurdle towards cooperation is that agents do not know how their behavior affects others. Specifically, agents neither receive any feedback on how their actions affect payoffs of fellow agents, nor on costs that they might induce to others. These factors are therefore external from the perspective of individual agents, as they are not considered in their individual reward functions. Moreover, there is no incentive for individual agents to internalize external costs as long as they are not being compensated or receive something in return. Combined, these aspects can diminish the overall reward as under such circumstances individual rational decision making will not necessarily lead to Pareto optimal results \cite{leibo2017multi}.

In this work, we propose to enrich mixed-motive scenarios with a market mechanism, to change the dynamics of the game through rules that generate incentives so as to turn cooperation into a dominant strategy. We argue that by entering mutual agreements via trades, returns of independent agents become interdependent, which helps to internalize former external costs (and profits).  We call a Stochastic Game extended by a market a Stochastic Market Game (SMG), which we formally define as a tuple: $(\mathcal{G}, \mathcal{A}_1^{m},...,\mathcal{A}_N^{m}, \mathcal M)$ consisting of 
\begin{itemize}
    \item The underlying Stochastic Game $\mathcal{G}$ with a set of states $S$, a set of environmental actions $\mathcal{A}_1^{e},...,\mathcal{A}_N^{e}$, the transition function $\mathcal P: S \times \mathcal{A}_1^{e} \times... \times \mathcal{A}_N^{e} \to PD(\mathcal S)$, and reward functions $r_{i}: \mathcal S \times \mathcal{A}_1^{e} \times...\times \mathcal{A}_N^{e} \to \mathbb{R}$ for each agent $i$.
    \item A collection of market action sets $\mathcal{A}_1^{m},...,\mathcal{A}_N^{m}$, one for each agent. 
    \item A market function $\mathcal M : \mathcal S \times \mathcal{A}_1^{m} \times...\times \mathcal{A}_N^{m} \times \mathbb{R}^{N} \to \mathbb{R}^{N}$, that computes the redistribution of rewards based on the state, agents' market actions, and rewards.
    % \item $P(....)$ state based price function??
 \end{itemize}
 
The Stochastic Market Game allows agents to become market participants by applying market actions $a^{m} \in \mathcal{A}^{m}_{i}$ in addition to their environmental actions $a^{e} \in \mathcal{A}^{e}_{i}$ (see Figure \ref{fig:SMG}). We differentiate two types of market functions $\mathcal M$, which we call \textbf{unconditional markets} and \textbf{conditional markets}. An unconditional market allows trades between two agents that are not constrained through further conditions. Therefore, agents connected via an unconditional trade need not commit to specific behavior, rules or norms, hence unconditional trading is a way to interconnect payoffs without restricting agents' individual behavior. In contrast, a conditional market defines a trade as a bilateral commitment between agent $i$ and agent $j$ to make a transaction that is triggered when a specified condition occurs, such as specific events, states, or certain behavior of fellow agents.  We build our definition of a market on the concept of idealized markets \cite{miller1988comparative} that define rules such that individual participants cannot violate property rights, deceive or cheat other agents, as these laws are enforced by the environment.

\begin{figure}[hbtp]
\centering
\includegraphics[width=0.34\textwidth]{img/market/shareholder_market.pdf}
\caption{Shareholder market: agents buy shares to participate in other agents' returns or sell shares to let others participate in their own return.}
\label{fig:shareholder-market}
\end{figure}


\subsection{Unconditional Markets}
Unconditional markets are inspired by the idea that in order to align agents' goals, they need to be enabled to let other agents participate in their own return. This is similar to a company, issuing shares from which shareholders earn a dividend. In such an agreement the shareholder is not required to fulfill any specific actions in order to receive the dividend, hence the market works unconditionally. Transactions in such a market require agents to decide on whether to buy shares from other agents and whether to sell their own shares to others at each step. In this work we will use the terms unconditional market and shareholder market (SM) synonymously. 

Formally in the shareholder market agent $i$'s market action $a^{m}_{i,t}$ at time $t$ specifies the willingness to sell to agent $j$ or buy from agent $j$ respectively (see Figure \ref{fig:shareholder-market}). If the buying request from $i$ coincides with a selling offer from $j$ (or vice-versa), the transaction is done and $i$ holds a share from $j$. From there on, the share lets $i$ participate in $j$'s return by a fixed dividend $d$. Optionally, shares can also have a price $p$ that must be paid for buying the share in the first place. However, such a price is not mandatory, since agents with high stakes will be willing to give their shares freely to make other agents shareholders of them to align their goals.

\subsection{Conditional Markets}
The conditional market is based on the idea of allowing agent $i$ to transfer reward to agent $j$ in direct response to $j$'s behavior. In this sense, a conditional market defines a contract of sale between a seller and a buyer side, similar to real world contracts where two persons agree on a payout when the contract conditions are met. Here we consider the case where contract conditions can be specified via the market actions $A_{i}^{m}$, and can be based either on the current state $s_{t}$ or on the environmental actions $a^{e} \in \mathcal{A}^{e}_{i}$ that are executed by agents. Again we define the environment as a trusted entity that verifies the specified conditions, so agents are prevented from cheating or breaking a contract. 

An instance of a conditional market where the conditions are based on agents' actions has been proposed by \cite{schmid2018action}, as a so called action market (AM). In an action market, agent $i$'s action $\Vec{a}_{i,t}$ at time $t$ comprises both, an environmental action $a_{i,t}^{\texttt{env}}$ and possibly an offer action $a_{i, j,t}^{\texttt{offer}}$ towards agent $j$. If $j$ happens to execute the suggested action at time $t$, i.e. if  $a_{j,t}^{\texttt{env}}$ equals $a_{i,j,t}^{\texttt{offer}}$, then a trade between $i$ and $j$ is established. In this case, $i$ is obliged to give a predetermined price $p$ in terms of reward to $j$. 

%A conditional market can mitigate inefficiencies if agents directly need to incentivize others such as described in the Coin game \cite{lerer2017maintaining,eccles2019imitation}, where two agents (red and blue) inhabit a world where different coins emerge from time to time. Coins are also either red or blue to indicate whether they belong to the red or the blue agent. If the red agent picks the coin that is intended for the blue agent, then the blue agent gets a reward of $-2$ while the red agent receives a reward of $+1$ (and vice versa). In case they only pick their own coins, the finder still gets a reward of $+1$ but no costs are imposed to the other. The Coin game therefore, describes a scenario where agents have external costs, which depend on the behavior of the other agent.

%To transform the Coin game into a Stochastic Market game, consider a matrix game version of the Coin game, modelled with two matrices, each representing one of the coin states (e.g. current coin is red or current coin is blue). Both agents have two actions to either take the current coin or leave it to the other agent. The payoffs are given in Figure \ref{fig:coin-game}, with expectations based on a fifty-fifty chance in case agents take the same action, assuming ties are broken randomly.

%The Coin game can be transformed into a corresponding Stochastic Market game by introducing actions sets $\mathcal{A}_{1}^{m} \times \mathcal{A}_{1} = \mathcal{A}_{2} \times \mathcal{A}_{2}^{m} = \{(\textit{env}, \textit{offer}) | \textit{env} \in \{1, 2\}, \textit{offer} \in \{0, 1, 2\}\}$, such that an $\textit{offer}$ is proposed to the other agent while action $\textit{env}$ is executed. The market functions $M_{i}$ can be defined to redistribute rewards each step, based on whether agents followed the suggested actions, i.e.:
%$$ M_1((e_{1}, o_{1}), (e_{2}, o_{2}), r^{1}) = r^{1} + p * \delta_{e_1,o_{2}} - p * \delta_{e_2,o_{1}}$$
%$$ M_2((e_{1}, o_{1}), (e_{2}, o_{2}), r^{2}) = r^{1} + p * \delta_{e_2,o_{1}} - p * \delta_{e_1,o_{2}}$$ where $\delta_{i,j}$ is the Kronecker delta with $\delta_{i,j} = 1$ for $i = j$ and $0$ else.


\subsection{Learning Market Games}
%As described earlier, a Stochastic Market game (SMG) extends a given multi-agent scenario with market actions to let agents trade and a market function that defines the redistribution based on the market behavior. 
We now describe the training procedure for $N$ independent learners combined with our market approach. Here, the training is defined for episodic tasks, where learning is done over the course of $E$ episodes, each comprising a maximum number of $T$ steps (pseudocode  given in Algorithm \ref{alg:ILM}). For the training with a market, the market function $\mathcal M$ is initialized at the beginning of the training and called after each environmental step. The market function $\mathcal M$ returns the adjusted rewards with respect to the trades between agents.

The principle of the market function is shown in Algorithm \ref{alg:market-function}. Agents can have either claims or liabilities towards other agents, which are accumulated during the course of an episode and recorded in a balance sheet $b_t \in \mathbb{R}^{N \times N} \subset s_t$. At each market step, the actual trades are computed on the basis of agent's buying and selling offers. These offers are stored in the selling matrix $S \in N\times N$ and the buying matrix $B \in N \times N$ respectively. The distinction between the action market and the shareholder market lies in the way buying and selling offers are defined. In the action market, a selling offer $a_{i,j}^{\texttt{sell}}$ from agent $i$ towards agent $j$ is represented by $i$'s environmental action, whereas a buying offer $a_{i,j}^{\texttt{buy}}$ from $i$ to $j$ is defined as the environmental action that $i$ is willing to buy from $j$, hence $a_{i,j}^{\texttt{buy}}, a_{i,j}^{\texttt{sell}} \in A^{e}$. In the shareholder market, the selling and buying offer do not specify terms for the transaction (unconditional), therefore represent a binary choice: $a_{i,j}^{\texttt{buy}}, a_{i,j}^{\texttt{sell}} \in \{0, 1\}$. 




In case agents can trade with all other agents at a given time step, the action space increases exponentially with the number of agents, since agents need to decide for all other agents whether they want to make a buying or a selling offer. For the action market, the increase is even larger than for the shareholder market, as all offers are conditioned on an action which increases the number of possible offers by the number of available environmental actions. However, in practice action spaces can be effectively limited, by either limiting the number of possible offers at a time or by applying offers to groups of agents. In this work, we allow agents to make a buying offer only towards a single agent in the action market, through which the increase in action space is only linear in the number of agents: $|\mathcal A| = |\mathcal A^{e}| + ((N-1) *\mathcal |A^{e}| * |A^{e}|)$. For the shareholder market we use a variant that we term broadcasting offers, which means that the selling offer has no designated recipient so an agent willing to sell accepts all offers at a each step. 

\begin{algorithm}
\caption{Independent Learning with Market}\label{alg:ILM}
  \begin{algorithmic}[1]
  \For{\textit{episode $e$ $\in$ $E$}}
        %\State $M \gets \textit{am}$ $|$ $\textit{sm}$\Comment{init. market} 
        \For{\textit{step $t$ $\in$ $T$}}
            \For{\textit{agent ${i}$ $\in$ $N$}}
                \State $\Vec{a}_{i,t} \sim \pi^{i}(s_{t}|\theta^{i})$\Comment{sample action}
            \EndFor
            \State $s_{t+1} \gets \mathcal P(\Vec{a}_{t}|s_t)$\Comment{episode step}
            \State $\Vec{r}_{t} \gets \mathcal \mathcal R(\Vec{a}_{t}|s_t)$\Comment{get rewards}
            \State $\Vec{r}_{t},  \gets \mathcal M(\Vec{a_{t}}, \Vec{r}_{t}, s_t)$\Comment{call market} 
            \For{\textit{agent ${i}$ $\in$ $N$}}
                %\State save $(\mathcal O^{i}(s_{t}), \Vec{a}_{i,t}, \mathcal O^{i}(s_{t+1}), \Vec{r}'_{i,t})$ 
                \State train $\theta^{i}$ based on $s_{t}, \Vec{a}_{i,t}, s_{t+1}, \Vec{r}_{i,t}$
            \EndFor
        \EndFor
    \EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
  \caption{Market Function}\label{alg:market-function}
  \begin{algorithmic}[1]
\Procedure{$\mathcal M(s_t, \Vec{a}_{t}, \Vec{r}_{t})$}{}
    \State $b_t \gets s_t$\Comment{get balance from current state}
    \State $S, B \gets 0_{N, N}$
    \For{\textit{agent ${i}$ in $N$}}
        \For{\textit{agent ${j}$ in $N \setminus i$ }} 
            \State $S_{i,j} \gets a_{i,j}^{\texttt{sell}}$\Comment{register sell}
            \State $B_{i,j} \gets a_{i,j}^{\texttt{buy}}$\Comment{register buy}
        \EndFor        
    \EndFor
    \State $T \gets S \wedge B$\Comment{compute trades}
    \State $\Vec{r}_{t} \gets$ set rewards w.r.t. to $T$, $b_t$ and $\Vec{r_t}$
    \State \Return $\Vec{r}_{t}$
\EndProcedure
\end{algorithmic}
\end{algorithm}



%computes trades on the basis of a suggested action from agent $i$ towards agent $j$, while a trade in a shareholder market is realized if a buy offer from $j$ for a share from $i$ coincides with a sell offer from $i$ in which case $j$ acquires a single share with value $d$ from $i$, that is added to $j$'s balance sheet as a liability towards $i$. The balance sheet $b$ can be computed by concatenating the selling and buying offers $S$ and $B$. 

%Internally, the action market works on the basis of an offer matrix $O \in \mathbf{N}^{N \times N}$ to track the current offers for all actions at step $t$. Action $\Vec{a}_{i,t}$ from agent $i$ comprises the environmental action $a_{i,t}^{\texttt{env}}$ and an offer action $a_{i,j,t}^{\texttt{offer}}$ for agent $j$ that is added to the current offer sheet $O$ in field $i,j$. When all offers are booked, the conditions for an actual trade are verified by comparing all offers $o_{i, j} \in O_{:,i}$ for agent $i$ with the actual performed action $a_{i,t}^{\texttt{env}}$. If offer $o_{i, j}$ equals action $a_{i,t}^{\texttt{env}}$, the price $p$ for this action is added to agent $j$'s balance sheet, which marks a liability towards agent $i$.


Moreover, agents can only make either a  single selling or a single buying offer at a time, which reduces the size of the action space to: $|\mathcal A| =  |\mathcal A^{e}| * |\{0, 1\}| *(N)$. The trades at time $t$ are computed by the logical conjunct of the selling offers with the buying offers. Afterwards, the rewards are computed with respect to the current trades and agents' accumulated paying obligations from earlier trades, that have not yet been settled. An agent is solvent, i.e. able to pay its liabilities, in case it has earned a positive reward. Otherwise, agents have a liability to another agent, which is settled whenever the agent becomes solvent. Note that there can arise situations where paying obligations cannot be settled during the course on an episode. Optionally, agents can be allowed to make debts by paying their liabilities even if they received a non-positive reward, i.e., $r_{i,t} \leq 0$.

%The shareholder market differs in that there is no need to track offers in terms of action suggestions. If a sell and a buy offer coincide at time $t$, the buyer $i$ acquires a single share with value $d$, which is added to the sellers balance sheet as a liability towards $i$. The balance sheet $B$ can then straightforwardly be computed by concatenating the selling and buying matrices $S$ and $B$. 



\begin{comment}
\begin{algorithm}
  \caption{Market Functions}\label{alg:action_market}
  \begin{algorithmic}[1]
\Procedure{$\texttt{ActionMarket}(\Vec{a}_{t}, \Vec{r}_{t}, s_t)$}{}
    \State $b \gets s_t$\Comment{get balance from current state}
    
    \For{\textit{agent ${i}$ in $N$}}
        \For{\textit{agent ${j}$ in $N \setminus i$}}
            \State $a_{i}^{\texttt{env}}, a_{j,i}^{\texttt{offer}} \gets \Vec{a}_{t,i}, \Vec{a}_{t,j}$
            %\State $a_{j,i}^{\texttt{offer}} \gets \Vec{a}_{t,j}$
            \If{$a_{i}^{\texttt{env}} == a_{j,i}^{\texttt{offer}}$}
                \State $b_{i,j} \gets p$\Comment{$j$ owes $i$}
            \EndIf
        \EndFor
    \EndFor
    \State $\Vec{r_t}' \gets$ set rewards w.r.t. to $b_t$ and $r_t$
    \State \Return $\Vec{r_{t}}'$
\EndProcedure
%\end{algorithmic}
%\end{algorithm}
\newline
%\begin{algorithm}
%  \caption{Shareholder Market}\label{alg:shareholder_market}
%  \begin{algorithmic}[1]
\Procedure{$\texttt{ShareholderMarket}(\Vec{a}_{t}, \Vec{r}_{t}, s_t)$}{}
    \State $b \gets s_t$\Comment{get balance from current state}
    \State $S, B \gets 0_{N, N}$\Comment{init. sells and buys} 
    \For{\textit{agent ${i}$ in $N$}}
        \State $a_{i}^{\texttt{sell}}, a_{i,j}^{\texttt{buy}} \gets \Vec{a}_{t, i}$
        \State $S_{i} \gets a_{i}^{\texttt{sell}}, B_{i, j} \gets a_{i, j}^{\texttt{buy}}$\Comment{register offers}
    \EndFor
    \State $B \gets S \oplus B * d$\Comment{compute trades}
    \State $\Vec{r_t}' \gets$ set rewards w.r.t. to $b_t$ and $r_t$
    \State \Return $\Vec{r_{t}}'$
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{comment}

\begin{comment}
\begin{table}[]
\centering
\begin{tabular}{l|c|c|}
\cline{2-3}
                               & Action 1           & Action 2           \\ \hline
\multicolumn{1}{|l|}{Action 1} & $R_1$, $R_2 - \alpha$ & $0$,  $\alpha$          \\ \hline
\multicolumn{1}{|l|}{Action 2} & $0$,  $\alpha$          & $R_1$, $R_2 - \alpha$ \\ \hline
\end{tabular}
\caption{Two player matrix game with variable conflict between agents ($\alpha$)}
\label{tab:matrix-game}
\end{table}
\end{comment}




%In this work, there was no limit for the acquisition of shares from other agents but a buying offer can only be given for a single agent at a time.

%Rather, an agent $i$ specifies during each step whether it is willing to buy from another agent $j$ and whether is willing to sell to any other agent. I.e., while for the buying action agents need to specify the addressee for the offer, the selling action can be understood as a general commitment to sell (or sell not) to any potential buyer. 

%Buying or selling shares results in no direct exchange of reward. The only motivation for selling is to align other agents' goals with the seller's individual goals. The buyer on the contrary acquires shares to participate in other agents return in case of positive returns with a fix dividend $d_{s}$.






==> Stochastic Market Games/content/5-evaluation.tex <==
\section{Experiments}\label{sec:evaluation}
In this section we evaluate the proposed market mechanisms in different two player matrix games before we extend the evaluation towards temporally and spatially extended domains where we evaluate with up to $16$ independent agents.

\subsection{Two Player Games} Our first analysis aims at answering the question of how the level of conflict between two players affects the overall outcome and how the proposed market can be utilized in order to resolve the conflict in such a scenario. To that end, we propose the two player \textbf{Conflict game}, depicted in Figure \ref{fig:matrix-game}, where each player faces the choice between two actions $C$ and $D$. The joint action (vector of actions from both players) $(i, j)$ with $i, j \in \{C, D\}$ yields a reward of $(x, y)$ as given in the respective cell of the matrix, where $x$ is the reward for player $1$ (column player) and $y$ is the reward for player $2$ (row player). The amount of conflict between the players in this game can be controlled by the parameter $\alpha$: For $\alpha = 0$ and with $R_1, R_2 > 0$, the players' goals are perfectly aligned, so they only face a coordination challenge, which means they need to choose the same action in order to receive a positive reward. However, for growing values of $\alpha$ the players' goals start to diverge as the column player increasingly becomes incentivized to prefer an uncoordinated outcome, i.e. when player $1$ chooses $C$ then player $2$ prefers $D$ and vice versa. Finally, for $\alpha > R_2$ their goals are completely opposing each other so each player will only receive a positive reward if the other player fails to do so, in which case there is no Nash-equilibrium in pure strategies.
\begin{comment}
\begin{figure}[hbtp]
\centering
\includegraphics[width=0.47 \textwidth]{img/market/coord-comp-all.pdf}
\caption{Q-learning in the Conflict game for varying conflict $\alpha$.}
\label{fig:market-dynamics}
\end{figure}
\end{comment}




\begin{figure}
\centering
     \subfloat[Conflict game \label{fig:matrix-game}]{
       \includegraphics[align=c,width=0.17\textwidth]{img/envs/coord-comp.pdf}
     }
     \hfill
     \subfloat[Overall reward \label{fig:rewards-matrix-game}]{%
       \includegraphics[align=c,width=0.29\textwidth]{img/market/coord-comp.pdf}
     }
     \caption{Independent Q-learning in the Conflict game for varying conflict $\alpha$.}
     \label{fig:market-dynamics}
\end{figure}


For the experiment we set $R_1 = 0.375$ and $R_2 = 2.625$, so $R_1 + R_2 = 3$. Note however, that depending on $\alpha$ the maximum achievable overall reward can be smaller than $3$, since due to the conflict between the players some loss of reward is unavoidable. We therefore indicate the maximum achievable reward corresponding to a specific value of $\alpha$ with a dashed line in Figure \ref{fig:rewards-matrix-game} (called Pareto frontier), which has a V-shape: for $0 < \alpha < 2 / (R_1 + R_2)$, the maximum overall reward decreases before at $\alpha = R_1 + R_2 / 2$ it starts to increase again, as at this point agent $2$ will get more reward in case of choosing action $(C, D)$ or $(D, C)$ than both players can get from choosing $(C, C)$ or $(D, D)$.

We now analyze the learning dynamics with and without market between two independent learners in this game. To that end two independent Q-learners were trained over $25$ independent runs for each level of conflict $\alpha$, where each run consisted of $4000$ consecutive steps (see Figure \ref{fig:rewards-matrix-game}). With standard Q-learning and in case of no market, the overall reward from both agents follows the shape of the Pareto frontier up to the point where the Pareto frontier increases again. At this point, the increasing conflict between the two players cannot be resolved by the agents since their goals diverge. This loss in overall reward can be mitigated by introducing the action market mechanism in the following way: agent's available action spaces are extended with additional actions to allow the transfer of reward, thus the action space is extended from $\{C, D\}$ to $\{(C,-), (C ,C), (C,D), (D,-), (D,C), (D,D)\}$, where the first component indicates the player's own action and the second component is the offer towards the other player ($(C,-), (D, -)$ refer to actions with no intended trade). As is shown in Figure \ref{fig:rewards-matrix-game}, the overall reward achieved with the same Q-learning configuration in the presence of a market is identical or close to the Pareto frontier for all levels of $\alpha$, which demonstrates how the market serves as a catalyst to align agents' increasingly diverging goals.

%\begin{figure}[hbtp]
%\centering
%\includegraphics[width=0.25\textwidth]{img/market/normal-form-game.pdf}
%\caption{}
%\label{fig:normal-form-game}
%\end{figure}

%\begin{figure}[hbtp]
%\centering
%\includegraphics[width=0.48 %\textwidth]{img/envs/matrix-games.pdf}
%\caption{Canonical two player matrix game social dilemmas.}
%\label{fig:SDs}
%\end{figure}

We now turn to a two player scenario, called the Iterated \textbf{Prisoner's Dilemma} shown in Figure \ref{fig:pd-env}, which poses a challenge to cooperative behavior, since in a one-shot game, where the game is only played once a rational player will choose the globally non-optimal action $D$ (defection) even though both players can be better off when they both choose to cooperate (denoted $C$). In an iterated version of the Prisoner's Dilemma cooperation might emerge based on reciprocity. However, standard reinforcement learning is unlikely to produce meaningful cooperation based on reciprocity, since it requires recursive reasoning about the consequences of one's own behavior on others, which is not part of model-free RL. This circumstance can be seen in Figure \ref{fig:rewards-pd}, where we show results from Q-learning for $4000$ consecutive steps of the iterated Prisoner's Dilemma averaged over $1000$ independent runs with returns normalized between $0$ and $1$. As is shown, independent Q-learning is likely to converge to the unique, non-optimal Nash-Equilibrium ($D,D$), indicated by the low level of overall reward. Through the extension with a market in the same way as before, the learned strategies by independent Q-learning can be improved towards optimal play, that is cooperative play in all games as is shown in Figure \ref{fig:rewards-pd}. Interestingly, for the iterated Prisoner's dilemma we noted that only a negative price helps to increase cooperation (here we used $p=-1.9$) in which case agents' strategies are consistently changed to mutual cooperation $(C, C)$ after approximately $500$ steps, thereby achieving the maximum reward.

\begin{comment}
\begin{figure}
\centering
    \subfloat[Prisoner's Dilemma \label{fig:results-PD}]{
       \includegraphics[width=0.18\textwidth]{img/returns/PD.pdf}
     }
     \subfloat[Chicken game \label{fig:results-CH}]{%
       \includegraphics[width=0.24\textwidth]{img/returns/CH.pdf}
     }
     \hfill
    \subfloat[Stag Hunt \label{fig:rewards-matrix-game}]{%
       \includegraphics[width=0.24\textwidth]{img/returns/SH.pdf}
     }
     \caption{Normalized ($0,1$) rewards from independent Q-learning in canonical matrix game social dilemmas}
     \label{fig:matrix-game-results}
\end{figure}
\end{comment}

%To visualize the change in the dynamics of the game, we inspect the Prisoner's dilemma by means of $\alpha$-Rank, a population based evaluation technique \cite{omidshafiei2019alpha}. The $\alpha$-Rank discrete time dynamics of the Prisoner's Dilemma with and without market are shown in Figure \ref{fig:alpha-rank}. In case of no market, there are two actions available ($C$, $D$) and the two graph nodes correspond to the situation where all individuals in the population play either cooperative or defective. The time the populations spend in each strategy is quantified as the mass of the stationary distribution in this node. Edges between nodes correspond to the fixation probabilities for state pairs, so edge directions indicate the flow of individuals from a strategy towards a fitter strategy. In the standard Prisoner's dilemma all probability mass is accumulated in $D$, which means that defection is the fittest strategy, with no chance for cooperative individuals to survive. This is in compliance with the Nash-equilibrium for the Prisoner's dilemma. The game dynamics change for the Prisoner's dilemma with market, where more probability mass is assigned to the trading strategies $DC, CD, CC, DD$, with the existence of circles, that include cooperative strategies. With respect to the results of independent Q-learning, these changes of the game dynamics are sufficient to direct the learning process towards the global optimum outcome.   

\begin{comment}
\begin{figure}[hbtp]
\centering
\includegraphics[width=0.35 \textwidth]{img/returns/SDs.pdf}
\caption{}
\label{fig:SDs}
\end{figure}
\end{comment}


\begin{figure}
\centering
     \subfloat[Prisoner's Dilemma \label{fig:pd-env}]{
       \includegraphics[align=c,width=0.17\textwidth]{img/envs/PD-env.pdf}
     }
     \hfill
     \subfloat[Overall reward \label{fig:rewards-pd}]{%
       \includegraphics[align=c,width=0.29\textwidth]{img/returns/PD.pdf}
     }
     \caption{Comparison of independent Q-learning in the Prisoner's Dilemma with and without market.}
     \label{fig:PD}
\end{figure}


\begin{comment}
\begin{figure}
\centering
    \subfloat[PD: no market \label{fig:alpha-rank-pd}]{%
       \includegraphics[width=0.23\textwidth]{img/returns/pd-no-trading.png}
     }
     \subfloat[PD with market \label{fig:alpha-rank-pd-market}]{%
       \includegraphics[width=0.23\textwidth]{img/returns/alpha_rank.png}
     }
     \caption{Discrete-time dynamics of the Prisoner's dilemma based on the $\alpha$-Rank Markov-Conley chain analysis.}
     \label{fig:alpha-rank}
\end{figure}
\end{comment}

%For the evaluation, we consider action markets (AM) and shareholder markets (SM). Additionally, we evaluate the original version of the game without markets, as an independent baseline.

%These scenarios confront learners with situations where conflicts of interests arise due to shared resources, which motivates agents to learn greedy or aggressive policies \cite{leibo2017multi}. To extend this class of problems 

%Since both domains feature shared resources with parameters to control the abundance of these resources, the settings are comparable to the Gathering game used in \cite{leibo2017multi}, where agents compete for available apples.

%\begin{figure}[hbtp]
%\centering
%\includegraphics[width=0.32 \textwidth]{img/envs/env.pdf}
%\caption{Testing domain for Stochastic Market games featuring a variable number of agents (blue triangles) which comes in two variants: (1) as \textit{Smartfactory} where agents follow individual production plans but need to share available machines and (2) as \textit{Refinery} where two types of agents compete for resources that can either be consumed or refined. Both variants of the domain feature partially conflicting goals between agents but differ in the way these goals are interconnected and thus require different forms of coordination.}
%\label{fig:envs}
%\end{figure}


\begin{figure}
     %\subfloat[Return 4 agents $\textit{SF}$ \label{fig:rewards-4-agents-sm}]{%
     %  \includegraphics[width=0.32\textwidth]{img/returns/eval-smartfactory-mar%kets-4-agents-return.pdf}
     %}
     %\hfill
     \subfloat[Return 8 agents $\textit{SF}$ \label{fig:rewards-8-agents-sm}]{
       \includegraphics[width=0.24\textwidth]{img/returns/eval-smartfactory-markets-8-agents-return.pdf}
     }
     %\hfill
     \subfloat[Return 16 agents $\textit{SF}$ \label{fig:rewards-16-agents-sm}]{%
       \includegraphics[width=0.24\textwidth]{img/returns/eval-smartfactory-markets-16-agents-return.pdf}
     }
    \hfill
    %\subfloat[Return 4 agents $\textit{RF}$ \label{fig:rewards-4-agents-r}]{%
    %   \includegraphics[width=0.32\textwidth]{img/returns/eval-refinement-marke%ts-4-agents-return.pdf}
     %}
     %\hfill
     \subfloat[Return 8 agents $\textit{RF}$ \label{fig:rewards-8-agents-r}]{%
       \includegraphics[width=0.24\textwidth]{img/returns/eval-refinement-markets-8-agents-return.pdf}
     }
     %\hfill
     \subfloat[Return 16 agents $\textit{RF}$ \label{fig:rewards-16-agents-r}]{%
       \includegraphics[width=0.24\textwidth]{img/returns/eval-refinement-markets-16-agents-return.pdf}
     }
     \caption{Normalized return from $20$ independent runs of the Smartfactory ($\textit{SF}$, a and b) and Refinery ($\textit{RF}$, c and d) for MADDPG (MAD), PPO and DQN without market and with either shareholder market (P+SM, D+SM) or action market (P+AM, D+AM).}
     \label{fig:rewards}
\end{figure}


\subsection{N-Player Games}
We now turn to more complex scenarios, which scale in the number of agents and are inspired by resource allocation problems, where agents follow individual goals but share limited resources (e.g. machines). The first domain, called \textbf{Smartfactory} (\textit{SF}), holds $m$ different machine types that are to be used by the agents. For every episode, each agent receives a task that is comprised of $n$ machines, i.e. an agent must activate all $n$ machines (by visiting them) before it is considered to be done. Rewards are sparse, i.e. they are only given to an agent whenever it has visited all machines that are part of its task. There are two parameters to fine-tune the potential conflict between agents: $t_{\text{inactive}}$ regulates the number of time steps that a machine is inactive after usage (and thus not usable by any other agent). Consequently, competition between agents increases with increasing $t_{\text{inactive}}$. The second parameter concerns the urgency or priority of an agent to fulfil its task, with two possible priorities (high or low). If an agent’s task is assigned high priority, that agent receives a higher reward $r_{\textit{high}}$ after completion than the agent assigned with the low-priority task (which receives a reward defined by $r_\textit{low}$). An increasing gap between $r_{\textit{high}}$ and $r_{\textit{low}}$ increases the potential benefit of coordination and cooperation between agents in terms of overall reward.

The second domain, called \textbf{Refinery} is inhabited by two types of agents, namely \emph{refining} and \emph{consuming} agents, which compete for a common resource. Furthermore, the resource appears in two different classes, i.e. unrefined and refined. The distinguishing feature of a refining agent and a consuming agent is that the refiner has the choice of either consuming the unrefined resource, which yields a relatively small reward $r^{\textit{low}}$, or to refine the resource, in which case it can no longer be consumed by himself. A consuming agent, on the other hand, cannot refine the raw resource but can only consume the already refined units, which gives a high reward $r^{\textit{high}}$ to the consuming agent. The dilemma in this scenario is that the overall return is maximal if all available resources are refined and subsequently consumed. However, as a refining agent cannot consume the refined good, it is individually rational to consume the raw resource to achieve at least a small reward. In all runs we set $r_{\textit{high}} = 5, r_{\textit{low}} = 1$  $t_{\text{inactive}} = 8$ in the Smartfactory and $r_{\textit{high}} = 5, r_{\textit{low}} = 0.02$ in the Refinery.

%Therefore, this parameter controls the abundance of machines as a shared resource. 

%Thus, this parameter controls the pay-off asymmetry between agents. Consequently, an

%The respawn rate in the Gathering domain serves the same function as $t_{\text{inactive}}$ in the Smartfactory environment: to control the abundance of a shared resource. Hence, the factory can be considered a Sequential Social Dilemma \cite{leibo2017multi}. 

%In the Smartfactory environment, the overall episode reward (i.e. the summed episode rewards of both agents) can be used as a measure of the spectrum between cooperative and competitive/defective behaviour: whenever the agent with $r_{\textit{low}}$ is willing to make compromises regarding its machine use, agents with $r_{\textit{high}}$ will be able to finish their tasks sooner, resulting in a higher overall return on average. When agents act out of pure self-interest however, the probability that agents with $r_{\textit{high}}$ will finish first decreases, resulting in a lower overall return in expectation.

%The refinery domain therefore resembles the \textit{Escape Room} game, which has been recently proposed by \cite{yang2020learning} to study a scenario where an agent needs to incentivize another agent to perform specific actions. In the escape room domain, two agents inhabit a world that features a target, a lever and a door. One of the agents has the goal to reach the target by passing the door. The door only opens when the other agent pulls the lever. Similar to the Smartfactory, the overall return in the refinery measures the the level of coordinated action between the two agent groups, as high rewards can only be achieved for a growing number of refined resources.




%\paragraph{Agents and Training} In this work, agents are implemented as self-interested, independent learners, i.e. agents do not exchange information with each other. However, the market mechanism may be seen as some form of a central controller, since it receives information from agents (in the form of trading actions) and redistributes rewards based on these actions, which can lead to the emergence of coordinated actions between agents. On a technical level, agents are represented either as Deep Q-Networks (DQN) \cite{mnih2015human} or on the basis of Proximal Policy Optimization (PPO) \cite{schulman1707proximal}. All training runs consist of $10000$ episodes, with episodes lasting for a maximum of $200$ steps. DQN agents' policy and target network consist of two fully-connected layers of size $32$ and $16$, with exponential linear units (ELUs) \cite{clevert2015fast} activation functions. During training, experience is stored in a replay buffer $E$ with a maximum capacity of $20000$ transitions. 

%The target network is updated every $500$ steps and training starts after an initial $200$ steps of simulation. Updates are done on the basis of a mini batch with size $64$. During training, exploration is encouraged through $\epsilon$-greedy action selection, where $\epsilon$ is linearly decayed to a minimum of $\epsilon = 0.1$. PPO agents consist of an actor and a critic network, with two hidden layers of size $32$ and tangens hyperbolicus (tanh) as activation function. The models are updated every $5000$ steps for $4$ epochs with a learning rate of $0.002$. For this work, hyperparameters for DQN and PPO have not been further optimized through extended optimization but rather manually tuned until a decent performance was achieved.

For the evaluation, we compare the settings: DQN and PPO without markets (Stochastic Game baseline), DQN and PPO with action market (AM) or shareholder market (SM). We also show results from the Multi-Agent Deep Deterministic Policy Gradient (MADDPG) algorithm \cite{lowe2017multi} as a baseline featuring a centralized critic. All settings were tested with $4$, $8$ and $16$ agents with the overall return from $8$ and $16$ agents displayed in Figure \ref{fig:rewards} (normalized overall return, averaged over $20$ independent runs). 

\begin{figure}[hbtp]
\centering
\includegraphics[width=0.34 \textwidth]{img/returns/return-dist-prices-new.pdf}
\caption{Market reward distribution for different price levels.}
\label{fig:distribution}
\end{figure}


In all settings, the highest reward is achieved when either the action market or shareholder market is available. Learning without markets cannot achieve any outcome that goes beyond the expected equilibrium outcome under self-interested optimization. We presume one reason for the difference in outcomes between DQN and PPO in combination with a market is due to the difference in the size of the action spaces, where it seems that DQN can cope more easily with the increased action space in both market forms. This is also underlined by the drop of performance of PPO combined with an action market, which has a comparatively larger action space than the shareholder market.


%However, there are differences in the outcome with regard to the combination of learner and market type. Overall, DQN converges faster and more stable than PPO. Interestingly, in the Smartfactory, DQN with action market (AM) becomes more stable for increasing numbers of agents. DQN+SM reaches near optimum results ($5$) for all numbers of agents. PPO+SM also reaches near optimum results but is less sample efficient, especially for higher numbers of agents. While DQN+AM becomes more stable with increasing numbers of agents, PPO+AM's performance decreases in both domains when more agents are considered. 

%Both domains, the Smartfactory and the Refinery, represent scenarios that render conflicts between the goals of agents. In the Smartfactory, if agent $i$ with a high priority task finishes its tasks first, the maximum overall return of $r=5$ is achieved. 

%An outcome is Pareto efficient, if no agent can be made better off without decreasing the payoff for at least another agent at the same time. To

To further analyze outcomes with respect to the distribution among agents and their overall efficiency, we visualize the distribution of the returns, grouped for agents according to their task priority and for different levels of prices (dividends) in Figure \ref{fig:distribution}. Each point $(x, y)$ comprises the share of the overall reward from agents with high priority $x$, and the reward share of agents with low priority $y$. For all tested prices, the outcomes are closer to the Pareto frontier (more efficient) in the presence of a market. Interestingly, the efficiency of outcomes decreases for higher price levels in case of a shareholder market, whereas the results are less affected by the price in the action market, which does not influence the division of the return as much as the price levels in a shareholder market. Finally, the dividend and price level influences the division of the return between agents with high and low priority tasks, such that higher prices lead to an increased share of the return being assigned to agents with low priority tasks.

%In contrast, if agent $j$ with low priority completes its task before $i$, the episode yields a return of $r=1$, which is not efficient, since both agents could be better off if they decided to priotize $i$'s task and divide the resulting reward such that $j$ receives at least $r_{j} = 1$. For more than two agents, an outcome is efficient if the sum of all individual returns  $r_{i}$ sums up to $R^{\textit{max}} = 5$. 



%\subsection{Discussion}
%The results reported in section \ref{sec:evaluation} show an increase of overall return when a given Markov game is transformed into a SMG that allows agents to redistribute reward through dedicated actions, under the terms of the specified market function. 


%In contrast to real world markets, there are no transaction costs for trading. 

%In order for markets to work however, it might become necessary to regulate them, just like in the real world. Although not explicitly analysed, regulation of an SMG could include the number of possible trades per episode, and agents' ability to make debts, i.e. making negative rewards through spending. Setting these parameters would lead to different levels of restriction for an SMG.

%\paragraph{Credit conservation}
%Problems arising with agents, which can generate reward (or money) out of nothing has been discussed in the context of market based approaches. \cite{miller1988comparative} describes the evolution of infinite loops that are generated by agents rewarding each other through the generation of money. These so-called parasites emerge consistently when the systems runs for long periods. In the early experiments for this work, no debt limits were set and we found that it rendered the learning of agents highly unstable, with high variance in outcomes. We found that the setting with the most stable learning dynamics is one with no limits for trades, but without the possibility to make debts, i.e. to generate reward. Rather, agents owe other agents by buying actions in the action market or selling shares in the shareholder market. These debts are only conserved on an episodic basis and are cancelled afterwards. The debts against other agents are compensated only in the event of positive rewards, which means an agent that gives credit to another agent is only reinforced for doing so if that agent proves to be a valuable investment.

%These loops can be avoided by introducing a conserved quantity that exhibits the possibility for mutual self-reinforcement. In market terms, the quantity can be understood as a locally-conserved currency that is used to pay for services such that non-productive loops will go broke, since they do not provide a valuable service to entities outside their own group. 



%\paragraph{Prices and Dividends}
%Prices in a market result from the interplay of demand and supply of a given good. In practice, prices can be determined by different mechanisms, such as auctions or order books. In this work, agents can make offers for either actions or shares of other agents with bids of a fixed amount $p$. In this sense, prices do not evolve or change as a consequence of supply and demand but are manually set as a market parameter. This approach allows all agents to buy and sell under the same conditions and is therefore different to the bid assignment strategy proposed for the Hayek machine \cite{baum1999toward}, where agents are assigned a fixed, random bid so that only agents with appropriate bids survive. As seen in Figure \ref{fig:distribution}, the price level is a critical parameter and influences both the overall efficiency of the outcome and the return distribution among agents. The pricing scheme therefore seems to be an interesting starting point for further analysis. In this regard, a mechanism that allows agents to pay (or receive) individual prices depending on the current state or on their expected reward could be considered.




==> Stochastic Market Games/content/6-conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this work we consider the problem of independent learning in mixed-motive games. To mitigate the inefficiencies from independent learning we propose a market mechanism, which we formally define as Stochastic Market Game (SMG), in order to allow agents to interact by means of the market (meta) game. Furthermore, two classes of markets are introduced, categorized by the way trades between agents are specified as either conditional or unconditional. We analyze markets in the Prisoner's Dilemma, where market changes the game dynamics to let independent Q-learning consistently achieve optimal, i.e. cooperative results. Furthermore, two variations of a more complex environment are used, where agents face the challenge of partially conflicting goals under the constraint of shared resources and we find that the proposed markets significantly increase overall and agent specific returns.


%Two state-of-the-art deep RL approaches (Deep-Q-Networks and Proximal Policy Optimization) are used for evaluation, which are both trained in the original Markov game and in the corresponding SMG. From the experiments, we find that the SMG formulation significantly improves the outcome in terms of generated overall return. In addition to the increase in overall return, we find that individual returns of agents are also higher on average. However, the division of the surplus critically  depends on the used price (or dividend) level in the market.

%A conditional market gives opportunity to make trades under the condition of specific prerequisites, such as the actions that are applied to let agents incentivize each other directly to perform specific actions or to reach specific states. An unconditional market, on the other hand, is inspired by stock markets where a trade does not include a direct service in return. Rather, it makes agents shareholders of each other, thereby participating in returns of agents for which they hold shares.


==> Stochastic Market Games/contents.tex <==
\input{content/0-abstract}
\input{content/1-introduction.tex}
\input{content/2-related-work.tex}
\input{content/3-background.tex}
\input{content/4-approach.tex}
\input{content/5-evaluation.tex}
\input{content/6-conclusion.tex}


